WIP: An Engaging Undergraduate Intro to Model Checking in Software Engineering Using TLA+

Background: In this paper, we present our initial efforts to integrate formal methods, with a focus on model-checking specifications written in Temporal Logic of Actions (TLA+), into computer science education, targeting undergraduate juniors/seniors and graduate students. Formal methods can play a key role in ensuring correct behavior of safety-critical systems, yet remain underutilized in educational and industry contexts. Aims: We aim to (1) qualitatively assess the state of formal methods in computer science programs, (2) construct level-appropriate examples that could be included midway into one's undergraduate studies, (3) demonstrate how to address successive "failures" through progressively stringent safety and liveness requirements, and (4) establish an ongoing framework for assessing interest and relevance among students. Methods: After starting with a refresher on mathematical logic, students specify the rules of simple puzzles in TLA+ and use its included model checker (known as TLC) to find a solution. We gradually escalate to more complex, dynamic, event-driven systems, such as the control logic of a microwave oven, where students will study safety and liveness requirements. We subsequently discuss explicit concurrency, along with thread safety and deadlock avoidance, by modeling bounded counters and buffers. Results: Our initial findings suggest that through careful curricular design and choice of examples and tools, it is possible to inspire and cultivate a new generation of software engineers proficient in formal methods. Conclusions: Our initial efforts suggest that 84% of our students had a positive experience in our formal methods course. Future plans include a longitudinal analysis within our own institution and proposals to partner with other institutions to explore the effectiveness of our open-source and open-access modules.

==> adhoc_course_survey.tex <==
% https://ctan.math.washington.edu/tex-archive/macros/latex/contrib/tabularray/tabularray.pdf
\begin{tblr}{width=\linewidth,colspec={|l|l|l|c|c|c|l|}}
\hline
Co&Institution&Dept&Number&Lev&Last&Tools\\\hline
\hline
ca&Queens U&CS&422/835&B&2019f&Alloy\\\hline
us&Texas State U&CS&5392&G&2023f&Alloy\\\hline
us&U Iowa&CS&5810&G&2022f&Alloy\\\hline
us&U North Carolina&CS&590/790&B&2023s&Alloy\\\hline
us&MIT&CS&6.512&G&2023s&Coq\\\hline
us&Portland State U&CECS&410/510&B&2021w&Coq\\\hline
us&U Michigan&CSE&498&G&2024w&Daphny\\\hline
us&UIUC&CS&476&G&2023f&Maude\\\hline
de&U Dortmund&CS&306&U&2021f&MC\\\hline
de&FAU&CS&151316&U&2023w&MC\\\hline
us&U Florida&ECE&5934&G&2022f&MC\\\hline
de&U Hamburg&CS&MAKS&U&2024w&MC\\\hline
de&U Marburg&CS&079-200&U&2019f&MC\\\hline
de&U Münster&CS&104450&B&2024w&MC\\\hline
us&Northeastern U&CS&4830/7485&B&2023f&nuXMV\\\hline
at&TU Graz&CS&705040&G&2021w&SLAM\\\hline
us&IA State U&CS&412/512&B&2023&SPIN\\\hline
us&U Florida&ECE&4701/5702&B&2022f&SPIN\\\hline
us&UC Merced&EECS&272&G&2019f&SPIN\\\hline
es&UDC&CS&VV&U&2024s&SPIN\\\hline
us&Columbia U&CS&4113&G&2023&TLA+\\\hline
us&Drexel U&CS&576&G&2020w&TLA+\\\hline
tr&Middle East Tech&CE&510&G&2022f&TLA+\\\hline
sg&Natl.\ U Singapore&CS&5232&G&2024s&TLA+\\\hline
us&U New Hampshire&CS&745&G&2021f&TLA+\\\hline
is&Reykjavik U&CS&219&U&2023s&Uppaal\\\hline
at&TU Wien&CS&185.291&G&2021s&Various\\\hline
us&UC Berkeley&EECS&219c&G&2024s&Various\\\hline
us&Yale U&CS&454/554&B&2020f&Various\\\hline
ch&EPFL&CS&550&G&2020f&Verilog\\\hline
ch&ETH&CS&263-2812&G&2024s&Z3\\\hline
ca&UBC&CS&513&G&2020s&Z3\\\hline
\end{tblr}

==> parkinglot.tex <==
\appendix

\subsection{Code Examples}

\TODO{omit some of the testing examples if short on space}

asdf

\input{snippets/snip-testing-adhoc}

asdf

\input{snippets/snip-testing-table}

asdf

\[
\forall \texttt{s} \in \textit{String} : \texttt{isPalindrome(s)} \Leftrightarrow (\texttt{s} = \texttt{s.reverse})
\]

asdf

\input{snippets/snip-testing-property}

asdf

\input{snippets/snip-testing-stateful-adhoc}

asdf

\input{snippets/snip-testing-stateful-jqwik}

asdf

\begin{shaded*}
\input{snippets/snip-tla-equations}
\end{shaded*}

asdf

\begin{shaded*}
\input{snippets/snip-tla-superheroes}
\end{shaded*}

asdf

\begin{shaded*}
\input{snippets/snip-tla-microwave}
\end{shaded*}

asdf

\begin{shaded*}
\input{snippets/snip-tla-counter}
\end{shaded*}




\subsection{Parking Lot}


Primarily, we engage undergraduates who have completed foundational courses, including Introduction to Programming, Data Structures, and Discrete Structures. Our approach builds on prior exposure to system correctness and automated testing, progressively introducing universally quantified properties that mirror functional requirements more closely. Starting with simple \TLAplus models for intuitive examples, like puzzles, students advance to modeling event-driven systems and systems with explicit concurrency, focusing on safety and liveness requirements. This progression not only helps students grasp formal specification and verification of dynamic and concurrent systems but also addresses concurrency issues like thread safety and deadlock avoidance.

Our methodology has been applied for the second time during the Spring 2024 semester to over 20 students, showing preliminary evidence of increased receptiveness and capability in applying formal methods practically. Students demonstrated enhanced conceptual understanding and a keener interest in software correctness, driven by the use of \TLAplus.

We argue that \TLAplus’s integration into software engineering courses marks a promising step in formal methods education, aligning academic efforts with industry expectations. We offer insights for educators on implementing similar approaches and suggest areas for further research, aiming to foster a new generation of software engineers proficient in formal methods.



% \begin{outline}
% \1 Mathematical and engineering fundamentals
%   \2 FND.mf.2 Basic logic (a, E)
%   \2 FND.mf.3 Proof techniques (a, E)
%   \2 FND.mf.7 Finite state machines and regular expressions (c, E)
%   \2 FND.ef.4 Systems development (k, E)
% \1 Professional practice
%   \2 PRF.psy.1 Dynamics of working in teams and groups (a, E)
%   \2 PRF.com Communication skills (a, E)
% \1   



% MAA.md.1
% Modeling principles (e.g., decomposition, abstraction,
% generalization, projection/views, and use of formal
% approaches) c E
% MAA.md.2
% Preconditions, postconditions, invariants, and design by
% contract c E
% MAA.md.3 Introduction to mathematical models and formal notation k E

% MAA.tm.2
% Behavioral modeling (e.g., state diagrams, use case analysis,
% interaction diagrams, failure modes and effects analysis, and
% fault tree analysis) a E

% MAA.af.2
% Analyzing correctness (e.g., static analysis, simulation, and
% model checking) a E


% REQ.rfd.1 Definition of requirements (e.g., product, project, constraints, c E
% 32
% system boundary, external, and internal)

% REQ.rfd.4
% Requirements characteristics (e.g., testable, unambiguous,
% consistent, correct, traceable, and priority) c E
% REQ.rfd.5
% Analyzing quality (nonfunctional) requirements (e.g., safety,
% security, usability, and performance) a E

% REQ.rfd.6 Software requirements in the context of systems engineering k E

% VAV.rev.3
% Static analysis (common defect detection, checking
% against formal specifications, etc.)



% \1 Quality attributes for software (QUA.cc.5, k E)
% \1 Formal requirements analysis (REQ.rv.6)
% \1 Security-related verification and validation (SEC.dev.5)
% \end{outline}


To address the learning objectives listed above, the proposed approach combines the following key ingredients. 
Figure~\ref{figure:COMP335CourseOutline} shows the resulting color-coded course outline.
\begin{figure}[htbp]
  \centering
  \includesvg[inkscapelatex=false, width = \columnwidth]{figures/COMP 335 Course Outline}
  \caption{COMP 335 course outline showing main topics (concepts, methods, and tools grouped by techniques), project deliverables, assessments, and in-class group activities}
  % https://docs.google.com/drawings/d/1VJ-k7Kkpl3bOqyG8LAKw79CAYdMZdfSw2G-OWNkOMxI/edit
  \label{figure:COMP335CourseOutline}
\end{figure}

\subsection{Text from course outline graphic}

Technique: Unit testing
Example-based
Table-driven
Property-based (stateless and stateful)

Technique: Model checking
Constraint-based systems
Event-driven systems
Explicitly concurrent systems

Technique: Runtime verification
Code instrumentation
Verification of event traces

Assessments
2 tests
3 quizzes

Project 0a: Software installation

Project 0b: GitHub and test-driven development

Project 1a: Unit testing using examples, tables, and stateless properties

Project 1b: Stateful testing with Jqwik

Project 2a: Elevator control logic (TLA+)

Project 2b: Bounded buffer with concurrent producers and consumers (TLA+)

3-4 group activities related to projects



\subsection{Supporting Materials}



\TODO{Discuss} matching courses from the \href{FME Education Course Database}{https://fme-teaching.github.io/courses/} maintained by the \href{Formal Methods Teaching Committee}{https://fme-teaching.github.io/}


\begin{figure}[htbp]
  \centering
\begin{tcolorbox}%[title=COMP 335 Course Effectiveness Survey]
\footnotesize
\begin{enumerate}
\item Conceptual Understanding: My understanding of the core concepts in formal methods is comprehensive.
\item Real-World Applications: I can effectively apply formal methods to solve real-world problems.
\item Verification and Validation Skills: I possess strong skills in software verification and validation using formal methods.
\item Familiarity with Specification Languages: I am well-versed in various formal specification languages.
\item Model Checking Proficiency: I have a solid grasp of model checking techniques within formal methods.
\item Perceived Value in Software Engineering: I recognize the importance and value of formal methods in software engineering.
\item Analytical Skill Enhancement: This course will significantly enhance my analytical skills in formal methods.
\item Practical Implementation of Concepts: I am confident in my ability to implement the concepts learned in this course in practical scenarios.
\item Awareness of Research Trends: I am informed about the latest research and developments in formal methods.
\item Critical Evaluation Skills: I am adept at critically analyzing various approaches in formal methods.
\item Collaboration and Teamwork: I am prepared to work collaboratively on formal methods projects.
\item Role in Academic and Professional Growth: I understand how formal methods are integral to my growth in computer science.
\item Awareness of Learning Challenges: I am cognizant of the challenges involved in mastering formal methods.
\item Alignment of Expectations and Course Content: My expectations align well with the course's objectives and structure.
\item Interest in Advanced Formal Methods: I am keen to delve deeper into advanced topics in formal methods.
\end{enumerate}
\end{tcolorbox}
  \caption{COMP 335 course effectiveness survey (5-point Likert scale) administered as a pretest during the first week and as a posttest during the last week of the 15-week semester}
  \label{figure:COMP335SurveyQuestions}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[scale=0.2275]{figures/COMP 335 Survey Labels.png}
  \hspace{1em}
  \includegraphics[scale=0.2]{figures/COMP 335 Pretest.png}
  \hspace{1em}
  \includegraphics[scale=0.2]{figures/COMP 335 Posttest.png}
  \caption{COMP 335 course effectiveness survey trend: pretest (n = 24) vs.\ posttest (n = 18; 82\% of final class roster)}
  \label{figure:COMP335SurveyTrend}
\end{figure}



% Google search query:
% \begin{verbatim}
% syllabus formal methods course \TLAplus site:.edu
% \end{verbatim}

% actual search 1: syllabus formal methods course "\TLAplus" site:edu -site:academia.edu
% 19 "relevant" results - included the most current ones

% actual search 2: syllabus "formal methods" course "model checking" site:edu -site:academia.edu after:2015
% 70 "relevant" results - need to review and decide which others to include

% actual search 3: universität  "veranstaltung" "formale methoden"  "model checking" site:de -site:academia.edu after:2019 -jahresbericht

% actual search 4: universität  modulhandbuch "formale methoden"  "model checking" site:de -site:academia.edu after:2019 -jahresbericht

\begin{comment}
\textbf{Preliminary Observations}
\begin{itemize}
%    \item We might want to limit the course-by-course table to courses where we found a detailed syllabus.
%    \item We might want to mention separately that many German-speaking universities have advanced undergrad and MS-level electives in formal methods with model checking, in some cases using \TLAplus.
    \item Possible story is that \TLAplus is actually underrepresented in the curricular landscape, and there is an opportunity to make it more prominent because of its effectiveness, as our preliminary results and some of the related work suggest.
    \item There is pretty strong evidence, whether known or not known, that there is emphasis on advanced treatment of these topics. 
    \item We often underestimate what students are able to do. They can do a lot with proper integration of foundations and prerequisites. 300-level is already a bit advanced, so we could explore doing something at the 272-level (end of their second year).
    \item It can be engaging, and with the right mathematical treatment, it can be taught. 
% DONE \item Maybe 264 is more important for developing logical principles than 272.
% DONE    \item Add column "last offered" or "offered recently".
%    \item SPIN seems prominent but last updated 2020, so diminishing in relevance, while \TLAplus is picking up steam/well maintained. Also need to classify the other options, such as Alloy, focusing on \emph{model checking}. https://spinroot.com/spin/whatispin.html
    \item Conjecture: With the right moves, we could teach this earlier.
    \item \TODO{THIS} Motivating narrative, take a position, emphasize importance for CS students' journey - opening statement that makes readers excited about this work.
\end{itemize}
\end{comment}


%\GKT{This table is lovely. Exactly what I was hoping we could construct. WE need to make this more analysis-friendly though. Can we get a proper spreadsheet (Google is fine for this) and put into a folder that also contains all the syllabi. Make sure the syllabus name contains university, department (almost always CS), and course number(s) in PDF format. Once it is ready, I can create an artifact that can be included in our own references upon acceptance (if the submission is blind).}

% \TODO{check how recent SPIN-based courses are and look for others based on NuSMV}
% \TODO{look for courses in the Anglosphere and in Castilian and German, then explain search method}
% \KL{AU, NZ, ZA: none}


%ACM DL search query \url{https://dl.acm.org/action/doSearch?AllField=position+paper+formal+methods+important+teaching}

%There are some very important papers here: \url{https://dl.acm.org/action/doSearch?AllField=teaching+formal+methods+sigcse}. Many are around the time of me finishing my PhD. LOL

%\GKT{Here is a chat with my good ole friend GPT4: \url{https://chat.openai.com/share/f8c40770-c5c8-47b8-b179-86ad45b47dd4}}

%\GKT{For a 4-page WIP paper, we must be economical when it comes to presentation. We will not have room for lengthy discussions about curicular details that we used in the UnoAPI paper (and book chapter).}

%\GKT{Before we do any curricular mapping, let's prioritize related work. None of this matters if we don't motivate why we're doing this with some actual papers and evidence.}


==> snippets/snip-testing-adhoc.tex <==
%234567890123456789012345678901234567890123456789012
\begin{javacode*}{firstnumber=1}
assertTrue(Palindrome.isPalindrome("radar"));
assertFalse(Palindrome.isPalindrome("lidar"));
\end{javacode*}

==> snippets/snip-testing-property.tex <==
%234567890123456789012345678901234567890123456789012
\begin{javacode*}{firstnumber=1}
@Property
boolean isPalindromeWorks(@ForAll final String s) {
  return isPalindrome(s) == new StringBuilder(s)
    .reverse().toString().equals(s);
}
\end{javacode*}

==> snippets/snip-testing-stateful-adhoc.tex <==
%234567890123456789012345678901234567890123456789012
\begin{javacode*}{firstnumber=1}
@Test void testFIFODiscipline() {
  final var value1 = "hello";
  final var value2 = "world";
  assertTrue(fixture.offer(value1));
  assertTrue(fixture.offer(value2));
  assertEquals(value1, fixture.poll());
  assertEquals(value2, fixture.poll());
  assertTrue(fixture.isEmpty());
}
\end{javacode*}

==> snippets/snip-testing-stateful-jqwik.tex <==
%234567890123456789012345678901234567890123456789012
\begin{javacode*}{firstnumber=1}
@Provide Arbitrary<ActionChain<SimpleQueue<String>>> 
  simpleQueueActions() {
    return ActionChain
      .<SimpleQueue<String>>startWith(
        () -> new FixedArrayQueue<String>(5)
      )
      .withAction(new OfferAction())
      .withAction(new PollAction());
}

@Property void checkSimpleQueue(
  @ForAll("simpleQueueActions") 
    final ActionChain<SimpleQueue<String>> chain) {
      chain.run();
}
\end{javacode*}

==> snippets/snip-testing-table.tex <==
%234567890123456789012345678901234567890123456789012
\begin{javacode*}{firstnumber=110}
val table =
  "string" | "result" |
  "a"      ! true |
  "ab"     ! false |
  "mom"    ! true |
  "kid"    ! false
  // ...

table |> ( (s, r) => assert(isPalindrome(s) == r) )
\end{javacode*}

==> snippets/snip-tla-counter.tex <==
\begin{tlatex}
\@x{ {\VARIABLES} shared ,\, state ,\, local ,\, lock}%
\@pvspace{8.0pt}%
% \@x{ vars \.{\defeq} {\langle} shared ,\, state ,\, local ,\, lock {\rangle}}%
% \@pvspace{8.0pt}%
% \@x{ RequireCorrectness \.{\defeq} {\FALSE}}%
% \@pvspace{8.0pt}%
% \@x{ ImplementTermination \.{\defeq} {\FALSE}}%
% \@x{ ImplementProgress \.{\defeq} {\FALSE}}%
% \@x{ ImplementLocking \.{\defeq} {\FALSE}}%
% \@pvspace{8.0pt}%
\@x{ N \.{\defeq} 5}%
\@x{ Threads \.{\defeq} 0 \.{\dotdot} ( N \.{-} 1 )}%
\@pvspace{8.0pt}%
% \@x{ TypeOK \.{\defeq}}%
% \@x{\@s{8.2} \.{\land} shared \.{\in} Nat}%
% \@x{\@s{8.2} \.{\land} {\DOMAIN} local \.{=} Threads}%
%  \@x{\@s{8.2} \.{\land} \A\, t \.{\in} Threads \.{:} local [ t ] \.{\in} 0
%  \.{\dotdot} N}%
% \@x{\@s{8.2} \.{\land} {\DOMAIN} state \.{=} Threads}%
% \@x{\@s{8.2} \.{\land} \A\, v \.{\in} Threads \.{:} state [ v ] \.{\in}}%
% \@x{\@s{16.4} \{\@w{fetch} ,\,\@w{store} ,\,\@w{done} \}}%
% \@x{\@s{8.2} \.{\land} lock \.{\in} 0 \.{\dotdot} N}%
% \@pvspace{8.0pt}%
\@x{ IsUnlocked \.{\defeq} lock \.{=} N}%
\@x{ Lock ( t ) \.{\defeq} {\IF} ImplementLocking}%
\@x{\@s{8.2} \.{\THEN} t \.{\in} Threads \.{\land} lock \.{'} \.{=} t}%
\@x{\@s{8.2} \.{\ELSE} {\UNCHANGED} {\langle} lock {\rangle}}%
\@x{ IsLockedBy ( t ) \.{\defeq} ImplementLocking \.{\implies}}%
\@x{\@s{8.2} t \.{\in} Threads \.{\land} lock \.{=} t}%
\@x{ Unlock \.{\defeq} {\IF} ImplementLocking}%
\@x{\@s{8.2} \.{\THEN} lock \.{'} \.{=} N}%
\@x{\@s{8.2} \.{\ELSE} {\UNCHANGED} {\langle} lock {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Init \.{\defeq}}%
\@x{\@s{8.2} \.{\land} shared \.{=} 0}%
 \@x{\@s{8.2} \.{\land} state \.{=} [ t \.{\in} Threads \.{\mapsto}\@w{fetch}
 ]}%
\@x{\@s{8.2} \.{\land} local \.{=} [ t \.{\in} Threads \.{\mapsto} 0 ]}%
\@x{\@s{8.2} \.{\land} IsUnlocked}%
\@pvspace{8.0pt}%
\@x{ Fetch ( t ) \.{\defeq}}%
\@x{\@s{8.2} \.{\land} state [ t ] \.{=}\@w{fetch}}%
\@x{\@s{8.2} \.{\land} IsUnlocked}%
 \@x{\@s{8.2} \.{\land} local \.{'} \.{=} [ local {\EXCEPT} {\bang} [ t ]
 \.{=} shared ]}%
 \@x{\@s{8.2} \.{\land} state \.{'} \.{=} [ state {\EXCEPT} {\bang} [ t ]
 \.{=}\@w{store} ]}%
\@x{\@s{8.2} \.{\land} Lock ( t )}%
\@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} shared {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Store ( t ) \.{\defeq}}%
\@x{\@s{8.2} \.{\land} state [ t ] \.{=}\@w{store}}%
\@x{\@s{8.2} \.{\land} IsLockedBy ( t )}%
\@x{\@s{8.2} \.{\land} shared \.{'} \.{=} local [ t ] \.{+} 1}%
 \@x{\@s{8.2} \.{\land} state \.{'} \.{=} [ state {\EXCEPT} {\bang} [ t ]
 \.{=}\@w{done} ]}%
\@x{\@s{8.2} \.{\land} Unlock}%
\@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} local {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Terminating \.{\defeq}}%
\@x{\@s{8.2} \.{\land} ImplementTermination}%
 \@x{\@s{8.2} \.{\land} \A\, t \.{\in} Threads \.{:} state [ t ]
 \.{=}\@w{done}}%
\@x{\@s{8.2} \.{\land} {\UNCHANGED} vars}%
\@pvspace{8.0pt}%
\@x{ Next \.{\defeq}}%
\@x{\@s{8.2} \.{\lor} \E\, t \.{\in} Threads \.{:} Fetch ( t )}%
\@x{\@s{8.2} \.{\lor} \E\, t \.{\in} Threads \.{:} Store ( t )}%
\@x{\@s{8.2} \.{\lor} Terminating}%
\@pvspace{8.0pt}%
\@x{ Progress \.{\defeq} ImplementProgress \.{\implies}}%
\@x{\@s{8.2} \A\, t \.{\in} Threads \.{:} {\WF}_{ state} ( Next )}%
\@pvspace{8.0pt}%
 \@x{ Spec \.{\defeq} Init \.{\land} {\Box} [ Next ]_{ vars} \.{\land}
 Progress}%
\@pvspace{8.0pt}%
\@x{ Correctness \.{\defeq} {\Diamond} ( RequireCorrectness \.{\implies}}%
\@x{\@s{8.2} ( shared \.{=} N \.{\land} IsUnlocked ) )}%
\end{tlatex}


==> snippets/snip-tla-equations.tex <==
\GKT{I like this. Way better than showing full code, which can be a supplemental material reference.}
\begin{tlatex}
\@x{ {\VARIABLES} x ,\, y}%
\@pvspace{8.0pt}%
\@x{ Init \.{\defeq}}%
\@x{\@s{8.2} \.{\land} x \.{\in} 0 \.{\dotdot} 100}%
\@x{\@s{8.2} \.{\land} y \.{\in} 0 \.{\dotdot} 100}%
\@pvspace{8.0pt}%
\@x{ Next \.{\defeq} {\UNCHANGED} {\langle} x ,\, y {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Solved \.{\defeq}}%
\@x{\@s{8.2} \.{\land} x \.{+} y \.{=} 10}%
\@x{\@s{8.2} \.{\land} x \.{-} y \.{=} 4}%
\@pvspace{8.0pt}%
\@x{ Unsolved \.{\defeq} {\lnot} Solved}%
\end{tlatex}


==> snippets/snip-tla-microwave.tex <==
\begin{tlatex}
\@x{ {\VARIABLES}}%
\@x{\@s{8.2} door ,\, radiation ,\, timeRemaining}%
\@pvspace{8.0pt}%
% \@x{ vars \.{\defeq} {\langle} door ,\, radiation ,\, timeRemaining {\rangle}}%
% \@pvspace{8.0pt}%
% \@x{ RequireSafety \.{\defeq} {\FALSE}}%
% \@x{ RequireLiveness \.{\defeq} {\FALSE}}%
% \@pvspace{8.0pt}%
% \@x{ ImplementStartSafety \.{\defeq} {\FALSE}}%
% \@x{ ImplementOpenDoorSafety \.{\defeq} {\FALSE}}%
% \@x{ ImplementProgress \.{\defeq} {\FALSE}}%
% \@pvspace{8.0pt}%
% \@x{ TypeOK \.{\defeq}}%
% \@x{\@s{8.2} \.{\land} door \.{\in} \{ CLOSED ,\, OPEN \}}%
% \@x{\@s{8.2} \.{\land} radiation \.{\in} \{ OFF ,\, ON \}}%
% \@x{\@s{8.2} \.{\land} timeRemaining \.{\in} Nat}%
% \@pvspace{8.0pt}%
% \@x{ MaxTime \.{\defeq} 60}%
% \@pvspace{8.0pt}%
% \@x{ Init \.{\defeq}}%
% \@x{\@s{8.2} \.{\land} door \.{\in} \{ OPEN ,\, CLOSED \}}%
% \@x{\@s{8.2} \.{\land} radiation \.{=} OFF}%
% \@x{\@s{8.2} \.{\land} timeRemaining \.{=} 0}%
% \@pvspace{8.0pt}%
\@x{ IncTime \.{\defeq}}%
\@x{\@s{8.2} \.{\land} radiation \.{=} OFF}%
\@x{\@s{8.2} \.{\land} timeRemaining \.{'} \.{=} timeRemaining \.{+} 1}%
\@x{\@s{8.2} \.{\land} timeRemaining \.{'} \.{\leq} MaxTime}%
\@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} door ,\, radiation {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Start \.{\defeq}}%
\@x{\@s{8.2} \.{\land} radiation \.{=} OFF}%
\@x{\@s{8.2} \.{\land} ImplementStartSafety \.{\implies} door \.{=} CLOSED}%
\@x{\@s{8.2} \.{\land} timeRemaining \.{>} 0}%
\@x{\@s{8.2} \.{\land} radiation \.{'} \.{=} ON}%
 \@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} door ,\, timeRemaining
 {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Cancel \.{\defeq}}%
\@x{\@s{8.2} \.{\land} radiation \.{'} \.{=} OFF}%
\@x{\@s{8.2} \.{\land} timeRemaining \.{'} \.{=} 0}%
\@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} door {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Tick \.{\defeq}}%
\@x{\@s{8.2} \.{\land} radiation \.{=} ON}%
\@x{\@s{8.2} \.{\land} timeRemaining \.{'} \.{=} timeRemaining \.{-} 1}%
\@x{\@s{8.2} \.{\land} timeRemaining \.{'} \.{\geq} 0}%
\@x{\@s{8.2} \.{\land} {\IF} timeRemaining \.{'} \.{=} 0}%
\@x{\@s{16.2} \.{\THEN} radiation \.{'} \.{=} OFF}%
\@x{\@s{16.2} \.{\ELSE} {\UNCHANGED} {\langle} radiation {\rangle}}%
\@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} door {\rangle}}%
\@pvspace{8.0pt}%
\@x{ OpenDoor \.{\defeq}}%
\@x{\@s{8.2} \.{\land} door \.{'} \.{=} OPEN}%
\@x{\@s{8.2} \.{\land} {\IF} ImplementOpenDoorSafety}%
\@x{\@s{16.2} \.{\THEN} radiation \.{'} \.{=} OFF}%
\@x{\@s{16.2} \.{\ELSE} {\UNCHANGED} {\langle} radiation {\rangle}}%
\@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} timeRemaining {\rangle}}%
\@pvspace{8.0pt}%
\@x{ CloseDoor \.{\defeq}}%
\@x{\@s{8.2} \.{\land} door \.{'} \.{=} CLOSED}%
 \@x{\@s{8.2} \.{\land} {\UNCHANGED} {\langle} radiation ,\, timeRemaining
 {\rangle}}%
\@pvspace{8.0pt}%
\@x{ Next \.{\defeq} IncTime \.{\lor} ... \.{\lor} CloseDoor}%
% \@x{\@s{8.2} \.{\lor} IncTime}%
% \@x{\@s{8.2} \.{\lor} Start}%
% \@x{\@s{8.2} \.{\lor} Cancel}%
% \@x{\@s{8.2} \.{\lor} OpenDoor}%
% \@x{\@s{8.2} \.{\lor} CloseDoor}%
% \@x{\@s{8.2} \.{\lor} Tick}%
\@pvspace{8.0pt}%
 \@x{ TickProgress \.{\defeq} ImplementProgress \.{\implies} {\WF}_{ vars} (
 Next )}%
\@pvspace{8.0pt}%
 \@x{ Spec \.{\defeq} Init \.{\land} {\Box} [ Next ]_{ vars} \.{\land}
 TickProgress}%
\@pvspace{8.0pt}%
\@x{ DoorSafety \.{\defeq} RequireSafety \.{\implies}}%
\@x{\@s{8.2} ( door \.{=} OPEN \.{\implies} radiation \.{=} OFF )}%
\@pvspace{8.0pt}%
\@x{ HeatLiveness \.{\defeq} ( radiation \.{=} ON ) \.{\leadsto}}%
\@x{\@s{8.2} ( RequireLiveness \.{\implies} radiation \.{=} OFF )}%
\end{tlatex}


==> snippets/snip-tla-superheroes.tex <==
\begin{tlatex}
\@x{ Ages \.{\defeq} {\langle} 6 ,\, 8 ,\, 10 {\rangle}}%
\@x{ Kids \.{\defeq} Permutation ( \{ Bryan ,\, Sean ,\, Tony \} )}%
\@x{ Heroes \.{\defeq} Permutation (}%
\@x{\@s{8.2} \{ Batperson ,\, Spiderperson ,\, Superperson \} )}%
\@pvspace{8.0pt}%
\@x{ Init \.{\defeq}}%
\@x{\@s{8.2} \.{\land} kids \.{\in} Kids}%
\@x{\@s{8.2} \.{\land} heroes \.{\in} \{ p \.{\in} Heroes \.{:}}%
 \@x{\@s{16.4} p [ 1 ] \.{=} Spiderperson \.{\land} p [ 2 ] \.{=} Superperson
 \}}%
\@pvspace{8.0pt}%
\@x{ Next \.{\defeq} {\UNCHANGED} {\langle} kids ,\, heroes {\rangle}}%
\@pvspace{8.0pt}%
\@x{ BryanLikesSpider \.{\defeq} \E\, i \.{\in} 1 \.{\dotdot} 3 \.{:}}%
 \@x{\@s{8.2} kids [ i ] \.{=} Bryan \.{\land} heroes [ i ] \.{=}
 Spiderperson}%
\@pvspace{8.0pt}%
 \@x{ TonyDoesntLikeSuper \.{\defeq} {\lnot} \E\, i\@s{8.2} \.{\in} 1
 \.{\dotdot} 3 \.{:}}%
\@x{\@s{8.2} kids [ i ] \.{=} Tony \.{\land} heroes [ i ] \.{=} Superperson}%
\@pvspace{8.0pt}%
\@x{ Solved \.{\defeq}}%
\@x{\@s{8.2} \.{\land} BryanLikesSpider}%
\@x{\@s{8.2} \.{\land} TonyDoesntLikeSuper}%
\@pvspace{8.0pt}%
\@x{ Unsolved \.{\defeq} {\lnot} Solved}%
\end{tlatex}

